Agile Robot Navigation through Hallucinated Learning and Sober Deployment

Learning from Hallucination (LfH) is a recent machine learning paradigm for autonomous navigation, which uses training data collected in completely safe environments and adds numerous imaginary obstacles to make the environment densely constrained, to learn navigation planners that produce feasible navigation even in highly constrained (more dangerous) spaces. However, LfH requires hallucinating the robot perception during deployment to match with the hallucinated training data, which creates a need for sometimes-infeasible prior knowledge and tends to generate very conservative planning. In this work, we propose a new LfH paradigm that does not require runtime hallucination -- a feature we call "sober deployment" -- and can therefore adapt to more realistic navigation scenarios. This novel Hallucinated Learning and Sober Deployment (HLSD) paradigm is tested in a benchmark testbed of 300 simulated navigation environments with a wide range of difficulty levels, and in the real-world. In most cases, HLSD outperforms both the original LfH method and a classical navigation planner.

==> content/approach_old.tex <==
\section{APPROACH}
\label{sec::approach}
In this section, we present our Hallucinated Learning and Sober Deployment (HLSD) technique for mobile robot navigation. We start with a simplified example, which assumes the robot to be a point mass, to illustrate the rationale behind hallucination for optimizing shortest path. We then present our hallucination strategy for a realistic non-holonomic mobile robot. To avoid hallucination at deployment time, we then introduce a sampling algorithm to create many C-spaces during training, where the actions performed in the open training environment is always optimal. 

\subsection{Point Robot Example}
\label{sec::point_robot}
We first present a simplified example, which assumes a point mass robot. In this case, the robot’s workspace is exactly the C-space. We use the same notation used by Xiao {\em et al}. to formalize LfH~\cite{xiao2021toward}: given a robot's C-space partitioned by unreachable (obstacle) and reachable (free) configurations, $C = C_{obst} \cup C_{free}$, 
% where $C_{obst} \in \mathcal{C}_{obst}$, 
the classical motion planning problem is to find a function $f(\cdot)$ that can be used to produce optimal plans $p=f(C_{obst}~|~c_c, c_g)$ that result in the robot moving from the robot's current configuration $c_c$ to a specified goal configuration $c_g$ without intersecting $C_{obst}$. Here, a plan $p \in \mathcal{P}$ is a sequence of low-level actions $\{u_i\}_{i=1}^{t}$ (i.e. $\mathcal{U}$ is the robot’s action space). Considering the ``dual" problem of finding $f(\cdot)$, the LfH includes a method to find the (unique) \emph{most constrained} unreachable set corresponding to $p$, $C_{obst}^*$. In this work, however, we introduce the definition of a (not unique) \emph{minimal} unreachable set, $C_{obst}^{min}$, corresponding to $p$:  
% \bo{the simplified definition is still problematic, we should focus on a single continuous curve from $c_m'$ to $c_m$ and nothing more. In fact according to current definition, $f(C_{obst}^{min} | c_c,c_g)$ not necessarily equals $p$. Consider we have two curves connecting $c_m'-c_m$, both overlap at beginning and end but are separate in middle. Then $C_{obst}^{min}$ has a hole in middle.}
% \begin{equation}
% \begin{gathered}
% C_{obst}^{min} = \{c\}_{i=1}^{\infty},~\text{s.t.}~\forall~c \in C_{obst}^{min},\\
% ~f(C_{obst}~|~c_c, c_g) = p,~f(C_{obst}\setminus c~|~c_c, c_g) \neq p
% \end{gathered}
% \end{equation}
% \begin{equation}
% \begin{gathered}
% C_{obst}^{min} = \{c \mid f(C_{obst}\setminus \{c\}~|~c_c, c_g) \neq p, c \in C\}.
% \end{gathered}
% \end{equation}

\begin{definition}
% \begin{equation}
% \begin{gathered}
$\mathcal{C}_{obst}^{min} = \{C_{obst}^{min} \mid \forall c \in C_{obst}^{min}, 
f(C_{obst}^{min}\setminus\{c\}~|~c_c, c_g) \neq f(C_{obst}^{min}~|~c_c,c_g)\}$
% \end{gathered}
% \end{equation}
\label{def::min}
\end{definition}
% Each element of $\mathcal{C}_{obst}^{min}$ is denoted as $C_{obst}^{min}$. 
In other words, $C_{obst}^{min}$ is the minimal set of obstacles that lead to $p$ being an optimal plan. 
In this work, we assume $C_{obst}^{min}$ to be connected (\textbf{connectivity assumption}), i.e. cannot be represented as the union of two disjoint nonempty open sets. 
Assuming $c_c$ and $c_g$ cannot be connected with a straight line of configurations which all belong to $C_{free}$ (there exists obstacle between $c_c$ and $c_g$), the base case (any other cases can be reduced to this case) of a robot path following an optimal plan $p$ to move from $c_c$ to $c_g$ is composed of configurations on two straight line segments, $c_c-c_m$ and $c_m-c_g$. The intermediate turning point is defined as $c_m$. Since $c_m$ is one configuration on the robot path resulted by $p$, we say $p$ \emph{goes through} $c_m$ (shown in Fig. \ref{fig::c_obst^min}). Here, we further assume there exists another symmetrical optimal plan $p'$ with respect to the line defined by $c_c$ and $c_g$, and goes through the reflection symmetry point of $c_m$, denoted as $c_m'$ (\textbf{symmetry assumption}). 
In the following, given a point-mass robot moving from $c_c$ to $c_g$ according to some optimal plan $p$ computed by $f(\cdot)$, we want to derive $\mathcal{C}_{obst}^{min}$ (\textit{\textbf{Definition} \ref{def::min}}), i.e. all minimum unreachable sets $C_{obst}^{min}$,  based on the \textbf{connectivity assumption} and \textbf{symmetry assumption}. 

% The following proposition follows immediately from the definition.
\begin{proposition}
If $c \in C_{obst}^{min}$, then the updated optimal plan $\hat{p} = f(C_{obst}^{min}\setminus \{c\}~|~c_c, c_g)$ must go through $c$.
\label{prop::1}
\end{proposition}
\begin{proof}
Assume $\hat{p}$ does not go through $c$, since for $C_{obst}^{min}\setminus\{c\}$, $\hat{p}$ is optimal, not $p$, adding $c$ back to $C_{obst}^{min}\setminus\{c\}$ does not affect the optimality of $\hat{p}$, this contradicting the assumption that $p$ is optimal for $C_{obst}^{min}$. 
\end{proof}
% It is trivial to show that if discarding $c$ will cause another optimal plan $\hat{p}$, then $\hat{p}$ must go through $c$.  
% In addition, we define the union of all minimum unreachable as $\mathcal{C}_{obst}^{min}$. 
% $C_{obst}^{min}\in\mathcal{C}_{obst}^{min}$. 

\begin{lemma}
The optimal plan $p=f(C_{obst}~|~c_c, c_g)$ optimizes for shortest-path $\Rightarrow$ $c_m\in C_{obst}^{min}$.\footnote{$C$ is a topological space, $C_{obst}$ is a closed set, and $C_{free}=C\setminus C_{obst}$ is an open set. $c_m$ is a boundary point of both $C_{obst}$ and $C_{free}$. The robot can come arbitrarily close to the obstacles while remaining in $C_{free}$~\cite{lavalle2006planning}.}
\label{lem::1}
\end{lemma}
\begin{proof} If $c_m \notin C_{obst}^{min}$, there is always an infinitesimal shorter path than the one executed by the optimal plan ($c_c \rightarrow c_m \rightarrow c_g$). 
\end{proof}
Based on the \textbf{symmetry assumption}, $c_m' \in C_{obst}^{min}$ as well. 
% \footnote{Technically, an accurate analytical representation (an ellipse whose focal points locate at $c_c$ and $c_g$, and semi-major axis is $(|c_c c_m'|+|c_m'c_g|)/2$ for the boundary $c_c-c_m'-c_g$ can be derived instead of simply using the symmetrical $c_m'$, but we introduce this assumption for simplicity.}
% Another special configuration is $c_m'$, which is the reflection symmetry point of $c_m$ with respect to the line connecting $c_c$ and $c_g$. 
Imagine a particular $C_{obst}^{\overline{min}}$ which contains all the configurations on the line connecting $c_m$ and $c_m'$ (shown in Fig. \ref{fig::c_obst^min} middle), discarding any $c$ in $C_{obst}^{\overline{min}}$ will result in a shorter path: $c_c \rightarrow c \rightarrow c_g$. 
% Due to the fact that $p=f(C_{obst}~|~c_c, c_g)$ is the optimal plan to move from $c_c$ to $c_g$, it is impossible to reach any configuration $c_n$ along the straight line connecting $c_m$ and $c_g$ or $c_n'$ along $c_m'$ and $c_g$ with a straight line. 
% In general, denote any configuration along the straight line connecting $c_m$ and $c_g$ and the straight line connecting $c_m'$ and $c_g$ as $c_n$ and $c_n'$, respectively, or $c_n^{(')}$ to refer to both, we have \bo{again, the lemma is true only if we consider simple continuous curves from $c_m'-c_m$. we should emphasize continuity again here}
% \begin{lemma}
% Given $p=f(C_{obst}~|~c_c, c_g)$, $\forall~c_n^{(')}$, $\nexists$ straight line path from $c_c$ to $c_n^{(')}$. 
% \end{lemma}
% This can be easily proved by contradiction: if there does exist a $c_n$ or $c_n'$ reachable from $c_c$ with a straight line, the optimal plan based on shortest-path principle is $c_c \rightarrow c_n^{(')}~(\neq c_m)\rightarrow c_g$. 
% \begin{proof}
% Assume $\exists~c_n^{(')}$ reachable from $c_c$ with a straight line, the optimal plan based on shortest-path principle then becomes $c_c \rightarrow c_n^{(')} \rightarrow c_g$ instead of $c_c \rightarrow c_m \rightarrow c_g$.
% \end{proof}

% Therefore, between $c_c$ and any $c_n^{(')}$), there must exist at least one $c \in C_{obst}$ (Fig. \ref{fig::c_obst^min} left). 
% \begin{lemma}
% Given $p=f(C_{obst}~|~c_c, c_g)$, $\forall~c_n^{(')}$, $\exists~c \in C_{obst}^{min}$ along the straight line between $c_c$ and $c_n^{(')}$. 
% \end{lemma}
% \begin{proof}
% Assume $\exists~c_n^{(')}$, s.t. between $c_c$ and $c_n^{(')}$, $\nexists~c \in C_{obst}^{min}$, the optimal plan based on shortest-path principle then becomes $c_c \rightarrow c_n^{(')} \rightarrow c_g$ instead of $c_c \rightarrow c_m \rightarrow c_g$.
% \end{proof}
\begin{lemma}
For any $c$ within the polygon $G$ defined by $c_c,c_m,c_g,c_m'$, there exists a $C_{obst}^{min}$ that contains $c$.
\label{lem::2}
\end{lemma}
\begin{proof}
For any $c \in G$, consider the $C_{obst}$ which consists of two line segments $c_m'-c-c_m$ ($C_{obst}^{min1}$ in Fig. \ref{fig::c_obst^min}), clearly $f(C_{obst}~|~c_c, c_g) = p$. Meanwhile, removing any $c' \in C_{obst}$ will result in a new path $c_c\rightarrow c'\rightarrow c_g$ shorter than the path $c_c\rightarrow c_m \rightarrow c_g$ induced by plan $p$. 
% To see this, WLOG, assume $c'$ is to the right of $c_c-c_g$. Connect the line from $c_c-c'$ and extend it until the line intersects $c_m-c_g$ at $c_z$. Then the path $c_c-c_m-c_g$ is longer than $c_c-c_z-c_g$, which is longer than $c_c-c'-c_g$ by triangle inequality. 
Hence, $C_{obst} \in \mathcal{C}_{obst}^{min}$.
\end{proof}
% The fact that there exists a straight line path from $c_n^{(')}$ to $c_g$ is guaranteed by the existence of optimal plan $p$ and the symmetry assumption. 
% Examples of possible $c \in C_{obst}$ are shown as black dots in the left of Fig. \ref{fig::c_obst^min}. The union of all these $c \in C_{obst}$ between $c_c$ and any $c_n^{(')}$ composes one instance of $C_{obst}^{min}$ (black lines). 

\begin{lemma}
Given $c \in C_{obst}^{min}$, $c$ must be confined within the polygon $G$ defined by $c_c$, $c_m$, $c_g$, and $c_m'$.
\label{lem::3}
\end{lemma}
\begin{proof}
Assume $\exists~c \in C_{obst}^{min}$ outside of $G$, due to the \textbf{connectivity assumption} and the existence of $c \in C_{obst}^{min}$ in the polygon, there must exist some consecutive configurations $c_b \in C_{obst}^{min}$ crossing the boundary. This contradicts the existence of optimal plan $p$ and $p'$.
% then there either exists straight line paths between $c_c$ and $c$ and between $c$ and $c_g$, or does not exist. For either cases, after discarding $c$ from $C_{obst}^{min}$, the optimal plan is still $p$. Therefore, $c \notin C_{obst}^{min}$. 
\end{proof}

% Note that (1) there exists $c \in C_{obst}^{min}$ along the straight line between $c_c$ and any $c_n^{(')}$ is only a necessary condition for $p$ to be optimal, not sufficient, and (2) an accurate analytical representation of the boundary on the $c_m'$ side is actually a half ellipse whose focal points locate at $c_c$ and $c_g$, and whose semi-major axis is $(|c_c c_m'|+|c_m'c_g|)/2$, instead of a simplified polygon. These two points are the reasons why the connectivity and symmetry assumptions are introduced. 

% Examples where the connectivity and symmetry assumptions break is shown in the right of the dashed line in Fig. \ref{fig::c_obst^min}: (1) $C_{obst}$ is disconnected, so even though there is at least one $c \in C_{obst}$ between $c_c$ and any $c_n^{(')}$, $p$ is not guaranteed to be optimal. (2) $c$ actually needs to be confined within the area defined by the half ellipse and the triangle, because any $c$ within the half ellipse will have a shorter $|c_cc|+|cc_g|$ than $|c_cc_m'|+|c_m'c_g|$. 

% Therefore, under these assumptions any \emph{connected} $C_{obst}^{min}$ must (1) include $c_m$ and $c_m'$, (2) contain configurations between $c_c$ and any $c_n^{(')}$, and (3) cannot contain any configurations outside the polygon defined by $c_c$, $c_m$, $c_g$, and $c_m'$: 
Therefore, under the \textbf{connectivity assumption} and \textbf{symmetry assumption}, any 
% \emph{connected} 
$C_{obst}^{min}$ per \textit{\textbf{Definition} \ref{def::min}} must (1) include $c_m$ and $c_m'$ (\textit{\textbf{Lemma} \ref{lem::1}}), (2) contain configurations within the polygon $G$ (\textit{\textbf{Lemma} \ref{lem::2}}), and (3) cannot contain any configurations outside $G$ (\textit{\textbf{Lemma} \ref{lem::3}}): 
\begin{theorem}
$\mathcal{C}_{obst}^{min}$ is the polygon $G$ defined by $c_c$, $c_m$, $c_g$, and $c_m'$. 
\end{theorem}
\begin{proof}
$\forall c \in G$, from \textit{\textbf{Lemma} \ref{lem::2}}, $c \in \mathcal{C}_{obst}^{min}$, so $G \subset \mathcal{C}_{obst}^{min}$. $\forall c \in \mathcal{C}_{obst}^{min}$, from \textit{\textbf{Lemma} \ref{lem::3}}, $c \in G$, so $\mathcal{C}_{obst}^{min} \subset G$. Hence, $\mathcal{C}_{obst}^{min} = G$.
\end{proof}
We abuse the notation such that a configuration $c \in \mathcal{C}_{obst}^{min}$ (instead of $C_{obst}^{min} \in \mathcal{C}_{obst}^{min}$). Intuitively, every $C_{obst}^{min}$ is a homeomorphism to $C_{obst}^{\overline{min}}$~\cite{lavalle2006planning}. 


In realistic scenarios, with high configuration resolution ($c_c$, $c_m$, $c_g$, and $c_m'$ are very close to each other) and real-world obstacle footprint (not arbitrarily small), the possibility of having disconnected $C_{obst}$ within $G$ is very low, which justifies the \textbf{connectivity assumption}. 
% As shown in Sec. \ref{sec::realistic_robot}, the connectivity and symmetry assumption hold in most cases when the configuration resolution becomes dense and $C_{obst}^{min}$ is instantiated in terms of discrete LiDAR range readings. 
% % The set of all minimum unreachable sets $\mathcal{C}_{obst}^{min}$ is shown in grey in Fig. \ref{fig::c_obst^min}. 
Note that an accurate analytical representation of the $\mathcal{C}_{obst}^{min}$ boundary on the $c_m'$ side is actually a half ellipse whose focal points locate at $c_c$ and $c_g$, and whose semi-major axis is $(|c_c c_m'|+|c_m'c_g|)/2$, instead of a simplified half polygon (triangle). As shown in the right of the dashed line in Fig. \ref{fig::c_obst^min}, $c$ actually needs to be confined within the area defined by the half ellipse and the triangle, because any $c$ within the half ellipse will have a shorter $|c_cc|+|cc_g|$ than $|c_cc_m'|+|c_m'c_g|$. But with high configuration resolution, the area of the half ellipse and triangle becomes small, whose difference becomes negligible. This justifies the \textbf{symmetry assumption}.

\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{content/figures/c_obst^min4.png}
  \caption{Left: 
%    Minimum unreachable set for a given plan is not unique, 
  $C_{obst}^{min_1},~C_{obst}^{min_2},~...,~C_{obst}^{\overline{min}} \in \mathcal{C}_{obst}^{min}$. 
%   but all minimum unreachable sets have certain properties in common: $c_m, c_m' \in C_{obst}^{min}$ and all $c \in C_{obst}^{min}$ are confined within the polygon defined by $c_c$, $c_m$, $c_g$, and $c_m'$. 
  Right: Actual $\mathcal{C}_{obst}^{min}$ without symmetry assumption. }
  \label{fig::c_obst^min}
\end{figure}

\subsection{Realistic Nonholonomic Robot}
\label{sec::realistic_robot}
Based on the principles discussed in Sec. \ref{sec::point_robot}, we present the hallucination technique for a realistic robot. In realistic scenarios, we approximate $\mathcal{C}_{obst}^{min}$ with $C_{obst}^{\overline{min}}$. 

A realistic robot cannot be modeled as a simple point mass: (1) the size is not negligible and (2) it cannot change motion direction instantly. The former causes a difference in the robot workspace and C-space, while the latter introduces nonholonomic motion constraints. To address (1), we define one point to the left and another to the right of the centroid of the robot, offset by the robot width, as footprint points, shown in Fig. \ref{fig::real_robot}. The instant linear velocity along the line between these two footprint points is zero for nonholonomic vehicles. The polygon defined by a sequence of footprint points belongs to the reachable set $C_{free}$. The actual path executed by the optimal plan $p$ locates in the middle of this area. To address (2), we define $c_{\omega}$ as configurations where the robot has a non-zero angular velocity ($\omega \neq0$). $c_{\omega}$ corresponds to the $c_m$ in the point mass case. Based on the sign of $\omega$, the robot turns left or right. We use the two boundaries defined by the sequence of footprint points to approximate $c_c \rightarrow c_m \rightarrow c_g$ in the point robot example. If the robot turns left ($\omega>0$) or right ($\omega<0$), the left or right boundary is chosen, respectively. For each triple of consecutive footprint points from the corresponding left or right boundary, whose middle point corresponds to a configuration with non-zero $\omega$, we treat them as $c_c$, $c_m$, and $c_g$ and perform the same operations as in Fig. \ref{fig::c_obst^min}. Since a real robot path is dense, the polygon defined by those points has a small area. Therefore we simply approximate all different $C_{obst}^{min}$ with $C_{obst}^{\overline{min}}$. In particular, we define an ``opposite'' function of $f(\cdot)$: 
$C_{obst}^{\overline{min}} = o(p~|~c_c, c_g)$
as the \emph{minimum} hallucination function\footnote{Note the inverse function $f^{-1}(\cdot)$ does not exist. Technically, $c_g$ can be uniquely determined by $p$ and $c_c$, but we include it as an input to $o(\cdot)$ for notational symmetry with $f(\cdot)$.}. This function finds $C_{obst}^{\overline{min}}$ based on the fact that  $p$ is an optimal plan. 

In addition to the small polygon area in the case of realistic robot model, because $C_{obst}^{min}$ is instantiated in terms of discrete LiDAR range readings, the difference between different $C_{obst}^{min}$ and $C_{obst}^{\overline{min}}$ further diminishes, as visualized in Fig. \ref{fig::real_robot}. We project all $C_{obst}^{\overline{min}}$ onto the corresponding LiDAR beams and mark them as obstacles. 
For each LiDAR beam, we define a minimum and a maximum range, which limit the possible range readings of this particular beam based on the optimal plan $p$. For the beams directly intersect any $C_{obst}^{\overline{min}}$, the minimum range is equal to the maximum range. For other beams, the minimum range is determined by the boundary, as configurations within the boundary must be in $C_{free}$. The maximum range is simply determined by the LiDAR, or manually pre-processed to a certain threshold. 
% A visualization of the LiDAR beams is shown in Fig. \ref{fig::real_robot}. 


\begin{figure}
  \centering
  \includegraphics[width=0.8\columnwidth]{content/figures/real_robot.png}
  \caption{Applying the point robot example to the realistic robot case: $C_{obst}^{min}$ is instantiated as the LiDAR beams whose minimum and maximum are equal (orange and yellow beams overlay). Due to high configuration resolution and discrete LiDAR beams, $C_{obst}^{\overline{min}}$ can efficiently approximate different $C_{obst}^{min}$. }
  \label{fig::real_robot}
\end{figure}

\subsection{Sampling between Min and Max Range}
\label{sec::sampling}
Given a LiDAR scan with a minimum and maximum range for each beam, a sampling strategy is devised to create many obstacle sets, $C_{obst}$, in which $p$ is optimal. The LiDAR beams with equal min and max values correspond to $C_{obst}^{\overline{min}}$, and are therefore fixed. Those are the reason why $p$ is optimal for shortest path. Other beams with different min and max values are called flexible beams, and their actual values are not crucial in determining if $p$ is optimal. 

Our sampling strategy aims at creating different range readings that (1) resemble real-world obstacles, and (2) respect uncertainty/safety. For (1), most real-world obstacles have a certain footprint, and their surface contribute to continuity among neighboring beams. Starting from the first flexible beam, a random range is sampled between min and max with a uniform distribution. Moving on to the neighboring beam, if it is a flexible beam, with a probability $\alpha$, we increase, or decrease, the previous range by a small random amount, and assign the value to the current beam. This is to simulate the continuity in neighbouring beams. With probability $1-2\alpha$, we start from scratch and randomly sample between this beam's min and max values. This is to simulate the scenarios where the next beam misses the current obstacle, and reaches another one or does not reach any obstacle at all. For (2), we added an offset value as a function of the optimal plan $p$ to the ranges, for example, based on the speed of $p$. The rationale is that faster motion is correlated with more uncertainty or less safety, therefore only when the obstacles are far away from the robot, the optimal planner is confident to accelerate. We also apply this offset to the fixed beams, because a good planner should not ``cut corners" aggressively. 

The entire HLSD pipeline is described in Alg. \ref{alg::sober}. The input to the algorithm is a random exploration policy $\pi_{rand}$ in open space, the minimum hallucination function $o(\cdot)$, a \emph{sampling count} of hallucinated $C_{obst}$ to be generated per raw data, the $offset(\cdot)$ function, the probability $\alpha$, and a parameterized planner $f_{\theta}(\cdot)$. For every data in $\mathcal{D}_{raw}$ collected using $\pi_{rand}$ in open space (line 2), we hallucinate $C_{obst}^{\overline{min}}$ (line 5) and generate the min and max values for every LiDAR beam (line 6). Lines 8--19 correspond to the sampling technique to generate random laser scans. We instantiate $C_{obst}$ as LiDAR readings $L$ and add it to $\mathcal{D}_{train}$ (line 20). This process is repeated \emph{sampling count} times for every data in $\mathcal{D}_{raw}$. Finally, we train $f_{\theta}(\cdot)$ with supervised learning (line 23). This hallucinated learning enables sober deployment with real perceived configuration $C_{obst}^{real}$ without runtime hallucination (Lines 25--26).

\begin{algorithm}[htbp]
 \caption{Hallucinated Learning and Sober Deployment}
 \begin{algorithmic}[1]
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 %\renewcommand{\algorithmicensure}{\textbf{Output:}}
 \REQUIRE $\pi_{rand}$, $o(\cdot)$, \emph{sampling count}, \emph{offset}($\cdot$), $\alpha$, $f_{\theta}(\cdot)$
\\\hrulefill
  \STATE // \textbf{Hallucinated Learning}
  \STATE collect motion plans $\{p, c_c, c_g\}$ from $\pi_{rand}$ in free space and form raw data $\mathcal{D}_{raw} = \{p, c_c, c_g\}$ 
  \STATE $\mathcal{D}_{train} \leftarrow \emptyset$
  \FOR {every $\{p, c_c, c_g\}$ in $\mathcal{D}_{raw}$}
  \STATE hallucinate $C_{obst}^{\overline{min}} = o(p~|~c_c, c_g)$
  \STATE generate LiDAR range $L_{min}$ and $L_{max}$ with $C_{obst}^{\overline{min}}$
    \FOR {iter = 1 : \emph{sampling count}}
    \STATE $L \leftarrow \emptyset$
    \STATE $l^1 \sim [l_{min}^1, l_{max}^1]$, $l^1 \leftarrow l^{1} + offset(p)$
    % sample $l^1$ uniformly between $l_{min}^1$ and $l_{max}^1$
    \STATE add $l^1$ to $L$, $l^{last}\leftarrow l^1$
    \FOR{i = 2 : $|L|$}
        \IF{$l_{min}^{i}==l_{max}^{i}$}
            \STATE $l^i \leftarrow l_{min}^{i} + offset(p)$
        \ELSE
            \STATE increase, decrease $l^{last}$ by a randomly selected small amount, or $l^i \sim [l_{min}^i, l_{max}^i]$, $l^i \leftarrow l^{i} + offset(p)$, 
            % sample uniformly between $l_{min}^i$ and $l_{max}^i$, 
            with probability $\alpha$, $\alpha$, and $1-2\alpha$, respectively, and assign to $l^i$
        \ENDIF
        \STATE make sure $l^i \in [l_{min}^i, l_{max}^i]$
        \STATE add $l_i$ to $L$, $l^{last}\leftarrow l^i$
    \ENDFOR
    \STATE $C_{obst} \leftarrow L$, add $\{C_{obst}, p, c_c, c_g\}$ to $\mathcal{D}_{train}$
    \ENDFOR
  \ENDFOR
%   \STATE sample $\mathcal{D}_{raw}$ to generate a larger training set $\mathcal{D}_{train} = \{C_{obst}, p, c_c, c_g\}$, where $p=f(C_{obst}~|~c_c, c_g)$
  \STATE train $f_{\theta}(\cdot)$ with $\mathcal{D}_{train}$ by minimizing the error $\mathbb{E}_{(C_{obst}, p, c_c, c_g) \sim \mathcal{D}_{train}} \big[ \ell(p, f_\theta(C_{obst}~|~c_c, c_g))\big]$
\\\hrulefill
  \STATE // \textbf{Sober Deployment} (each time step)
  \STATE receive $C_{obst}^{real}, c_c, c_g$
  \STATE plan $p = \{u_i\}_{i=1}^{t} = f_{\theta}(C_{obst}^{real}~|~c_c, c_g)$
 \RETURN $p$
 \end{algorithmic}
 \label{alg::sober}
 \end{algorithm}




==> content/approach_old2.tex <==
\section{APPROACH}
\label{sec::approach}
% In this section, we present our Hallucinated Learning and Sober Deployment (HLSD) technique for mobile robot navigation. We start with a simplified example, which assumes the robot to be a point mass going through three consecutive non-colinear configurations, to illustrate the rationale behind hallucination for optimizing shortest path. We then present our hallucination strategy for a realistic non-holonomic mobile robot. This hallucination strategy produces all obstacles that are required for a motion plan to be optimal. To avoid hallucination at deployment time, we then introduce a sampling algorithm for other obstacles irrelevant to the plan's optimality to create many C-spaces during training, so the actions performed in the open training environment is optimal. 

In this section, we present our Hallucinated Learning and Sober Deployment (HLSD) technique for mobile robot navigation. In Sec. \ref{sec::point_robot}, we start with a simplified example, which assumes the robot to be a point mass that follows a relatively simple path, to introduce the idea of a minimal unreachable set, $C_{obst}^{min}$, for a given plan, and provide analysis of the family of all unreachable sets, $\mathcal{C}_{obst}^{min}$. In Sec. \ref{sec::realistic_robot}, we show how we use one single member of the minimal unreachable set family, $C_{obst}^{\overline{min}}$, to represent all members in the family. We also present how we adapt the point mass example to deal with real-world robots. In Sec. \ref{sec::sampling}, we introduce a sampling method to generate augmentations to the representative minimal unreachable set to cover the full set of configurations the planner needs to address during sober deployment. 

\subsection{Point Robot Example}
\label{sec::point_robot}
We first present a simplified example, which assumes a point mass robot going through three non-colinear configurations. In this case, the robot’s workspace is exactly the C-space. We use the same notation used by Xiao {\em et al}. to formalize LfH~\cite{xiao2021toward}: given a robot's C-space partitioned by unreachable (obstacle) and reachable (free) configurations, $C = C_{obst} \cup C_{free}$, 
% where $C_{obst} \in \mathcal{C}_{obst}$, 
the classical motion planning problem is to find a function $f(\cdot)$ that can be used to produce optimal plans $p=f(C_{obst}~|~c_c, c_g)$ that result in the robot moving from the robot's current configuration $c_c$ to a specified goal configuration $c_g$ without intersecting $C_{obst}$. Here, a plan $p \in \mathcal{P}$ is a sequence of low-level actions $\{u_i\}_{i=1}^{t}$ (i.e. $\mathcal{U}$ is the robot’s action space). Considering the ``dual" problem of finding $f(\cdot)$, LfH includes a method to find the (unique) \emph{most constrained} unreachable set corresponding to $p$, $C_{obst}^*$. In this work, however, we introduce the definition of a (not unique) \emph{minimal} unreachable set, $C_{obst}^{min}$, corresponding to $p$:  
% \bo{the simplified definition is still problematic, we should focus on a single continuous curve from $c_m'$ to $c_m$ and nothing more. In fact according to current definition, $f(C_{obst}^{min} | c_c,c_g)$ not necessarily equals $p$. Consider we have two curves connecting $c_m'-c_m$, both overlap at beginning and end but are separate in middle. Then $C_{obst}^{min}$ has a hole in middle.}
% \begin{equation}
% \begin{gathered}
% C_{obst}^{min} = \{c\}_{i=1}^{\infty},~\text{s.t.}~\forall~c \in C_{obst}^{min},\\
% ~f(C_{obst}~|~c_c, c_g) = p,~f(C_{obst}\setminus c~|~c_c, c_g) \neq p
% \end{gathered}
% \end{equation}
% \begin{equation}
% \begin{gathered}
% C_{obst}^{min} = \{c \mid f(C_{obst}\setminus \{c\}~|~c_c, c_g) \neq p, c \in C\}.
% \end{gathered}
% \end{equation}

\begin{definition}
% \begin{equation}
% \begin{gathered}
$\mathcal{C}_{obst}^{min} = \{C_{obst}^{min} \mid \forall c \in C_{obst}^{min}, 
f(C_{obst}^{min}\setminus\{c\}~|~c_c, c_g) \neq f(C_{obst}^{min}~|~c_c,c_g)\}$
% \end{gathered}
% \end{equation}
\label{def::min}
\end{definition}
% Each element of $\mathcal{C}_{obst}^{min}$ is denoted as $C_{obst}^{min}$. 
In other words, $C_{obst}^{min}$ is a minimal set of obstacles that lead to $p$ being an optimal plan. 
% In this work, we assume $C_{obst}^{min}$ to be connected (\textbf{connectivity assumption}), i.e. cannot be represented as the union of two disjoint nonempty open sets. 
Assuming $c_c$ and $c_g$ cannot be connected with a straight line of configurations which all belong to $C_{free}$ (there exists an obstacle between $c_c$ and $c_g$), the simplest case of a robot path following an optimal plan $p$ to move from $c_c$ to $c_g$ is composed of configurations on two straight line segments, $c_c-c_m$ and $c_m-c_g$. The intermediate turning point is defined as $c_m$. Since $c_m$ is one configuration on the robot's path, we say $p$ \emph{goes through} $c_m$ (shown in Fig. \ref{fig::c_obst^min}). 
% Here, we further assume there exists another symmetrical optimal plan $p'$ with respect to the line defined by $c_c$ and $c_g$, and goes through the reflection symmetry point of $c_m$, denoted as $c_m'$ (\textbf{symmetry assumption}). 
In the following, given a point-mass robot moving from $c_c$ to $c_g$ according to some optimal plan $p$ computed by $f(\cdot)$, we want to derive $\mathcal{C}_{obst}^{min}$ (\textit{\textbf{Definition} \ref{def::min}}), i.e. the set of all minimal unreachable sets $C_{obst}^{min}$. 

We name the union of all robot configurations in the triangle defined by $c_c$, $c_m$, and $c_g$ as $G_1$. On the other side of line $c_c-c_g$, we name the union of all configurations in the half ellipse, whose focal points locate at $c_c$ and $c_g$, and whose semi-major axis is $(|c_c c_m|+|c_mc_g|)/2$, as $G_2$. We define $G = G_1 \cup G_2$ (the grey area in Fig. \ref{fig::c_obst^min}). The purpose of Sec. \ref{sec::point_robot} is to show that every configuration in $G$ is in \emph{some} minimal unreachable set, and no configuration outside $G$ is in \emph{any} unreachable set, i.e. $\mathbf{\mathcal{C}_{obst}^{min} = G}$. \footnote{We abuse the notation such that a configuration $c \in \mathcal{C}_{obst}^{min}$ (instead of $C_{obst}^{min} \in \mathcal{C}_{obst}^{min}$). } 

% based on the \textbf{connectivity assumption} and \textbf{symmetry assumption}. 

% The following proposition follows immediately from the definition.
\begin{proposition}
If $c \in C_{obst}^{min}$, then the updated optimal plan $\hat{p} = f(C_{obst}^{min}\setminus \{c\}~|~c_c, c_g)$ must go through $c$.
\label{prop::1}
\end{proposition}
\begin{proof}
Assume $\hat{p}$ does not go through $c$, since for $C_{obst}^{min}\setminus\{c\}$, $\hat{p}$ is optimal, not $p$, adding $c$ back to $C_{obst}^{min}\setminus\{c\}$ does not affect the optimality of $\hat{p}$, this contradicting the assumption that $p$ is optimal for $C_{obst}^{min}$. 
\end{proof}
% It is trivial to show that if discarding $c$ will cause another optimal plan $\hat{p}$, then $\hat{p}$ must go through $c$.  
% In addition, we define the union of all minimal unreachable as $\mathcal{C}_{obst}^{min}$. 
% $C_{obst}^{min}\in\mathcal{C}_{obst}^{min}$. 

\begin{lemma}
The optimal plan $p=f(C_{obst}~|~c_c, c_g)$ optimizes for shortest-path $\Rightarrow$ $c_m\in C_{obst}^{min}$.\footnote{$C$ is a topological space, $C_{obst}$ is a closed set, and $C_{free}=C\setminus C_{obst}$ is an open set. $c_m$ is a boundary point of both $C_{obst}$ and $C_{free}$. The robot can come arbitrarily close to the obstacles while remaining in $C_{free}$~\cite{lavalle2006planning}.}
\label{lem::1}
\end{lemma}
\begin{proof} If $c_m \notin C_{obst}^{min}$, there is always an infinitesimal shorter path than the one executed by the optimal plan ($c_c \rightarrow c_m \rightarrow c_g$). 
\end{proof}
% Based on the \textbf{symmetry assumption}, $c_m' \in C_{obst}^{min}$ as well. 

% Imagine a particular $C_{obst}^{\overline{min}}$ which contains all the configurations on the line connecting $c_m$ and $c_m'$ (shown in Fig. \ref{fig::c_obst^min} middle), discarding any $c$ in $C_{obst}^{\overline{min}}$ will result in a shorter path: $c_c \rightarrow c \rightarrow c_g$. 



\begin{lemma}
For any $c$ within $G$, there exists a $C_{obst}^{min}$ that contains $c$.
\label{lem::2}
\end{lemma}
\begin{proof}
For any $c \in G$, for all  configurations along the line $c_m-c$. Only two possibilities exist: 

(1) If all configurations fall in $G$, then extend the line $c_m-c$ until it intersects the half ellipse boundary at $c_e$. Consider $C_{obst}$ which consists of all configurations on $c_m-c_e$, clearly, $f(C_{obst}~|~c_c, c_g) = p$ (based on the definition of ellipse, $|c_cc_e|+|c_ec_g|=|c_cc_m|+|c_mc_g|$). Meanwhile, removing any $c' \in C_{obst}$ will result in a new path $c_c\rightarrow c'\rightarrow c_g$ shorter than the path $c_c\rightarrow c_m \rightarrow c_g$ induced by plan $p$. Hence, $C_{obst} \in \mathcal{C}_{obst}^{min}$ (example shown as $C_{obst}^{min_1}$ in Fig. \ref{fig::c_obst^min}).

(2) If not all configurations fall in $G$, extend $c_g-c$ and intersects the half ellipse at $c_e$. Consider the $C_{obst}$ which consists of all configurations on lines $c_m-c_g-c_e$, clearly, $C_{obst} \in \mathcal{C}_{obst}^{min}$ (example shown as $C_{obst}^{min_2}$ in Fig. \ref{fig::c_obst^min}).

In both cases, $C_{obst} \in \mathcal{C}_{obst}^{min}$.
\end{proof}


\begin{lemma}
Given $c \in C_{obst}^{min}$, $c$ must be confined in $G$.
\label{lem::3}
\end{lemma}

\begin{proof}
Assume $\exists~c \in C_{obst}^{min}$ outside of $G$, only two possibilities exist: 

% (1) $c$ is in the left half plane defined by $c_c-c_g$: based on \textit{\textbf{Proposition} \ref{prop::1}}, $\hat{p} = f(C_{obst}^{min}\setminus \{c\}~|~c_c, c_g)$ must go through $c$. The shortest path which goes through $c$, if exisits, is $c_c-c-c_g$. However, based on the definition of ellipse, for any $c$ outside the ellipse, $|c_cc|+|cc_g|>|c_cc_m|+|c_mc_g|$. 

(1) $c$ is outside the entire (left and right half) ellipse: based on \textit{\textbf{Proposition} \ref{prop::1}}, the updated optimal plan $\hat{p} = f(C_{obst}^{min}\setminus \{c\}~|~c_c, c_g)$ must go through $c$. The shortest possible path, which goes through $c$, is $c_c-c-c_g$, if it exists. However, based on the definition of ellipse, for any $c$ outside the ellipse, $|c_cc|+|cc_g|>|c_cc_m|+|c_mc_g|$. This contradicts optimal $\hat{p}$. 

(2) $c$ is inside the entire ellipse, but outside $G$: $c$ must be in the right half of the ellipse but outside the triangle defined by $c_c$, $c_m$, and $c_g$ (Fig. \ref{fig::c_obst^min} right). Again, $\hat{p}$ must go through $c$. The shortest possible path which goes through $c$ is $c_c-c-c_g$, if it exists, which must intersect either $c_c-c_m$ or $c_m-c_g$ at some point $c_i$. Due to the substructure optimality of the shortest path $c_c-c_m-c_g$, the shortest path between any points on this shortest path must be its substructure. If $c_i$ is on $c_c-c_m$, then the shortest path from $c_i$ to $c_g$ must be $c_i-c_m-c_g$. $c_c-c-c_i-c_m-c_g$ is longer than $c_c-c_m-c_g$, and therefore not optimal. If $c_i$ is on $c_m-c_g$, the shortest path between $c_c$ and $c_i$ must be $c_c-c_m-c_i$. $c_c-c_m-c_i-c-c_g$ is longer than $c_c-c_m-c_g$, and therefore not optimal. In both cases, the shortest possible path going through $c$ is longer than $c_c-c_m-c_g$. This contradicts optimal $\hat{p}$. 

For both case (1) and (2), $c$ must be in $G$. 
% if $c$ is outside of $G$, clearly $c \notin C_{obst}^{min}$, because removing $c$ from $C_{obst}^{min}$ will not affect the optimality of $p$. 
\end{proof}

Therefore, any $C_{obst}^{min}$ per \textit{\textbf{Definition} \ref{def::min}} must (1) include $c_m$ (\textit{\textbf{Lemma} \ref{lem::1}}), (2) contain configurations within the polygon $G$ (\textit{\textbf{Lemma} \ref{lem::2}}), and (3) cannot contain any configurations outside $G$ (\textit{\textbf{Lemma} \ref{lem::3}}): 
\begin{theorem}
$\mathcal{C}_{obst}^{min}$ is $G$. 
\end{theorem}
\begin{proof}
$\forall c \in G$, from \textit{\textbf{Lemma} \ref{lem::2}}, $c \in \mathcal{C}_{obst}^{min}$, so $G \subset \mathcal{C}_{obst}^{min}$. $\forall c \in \mathcal{C}_{obst}^{min}$, from \textit{\textbf{Lemma} \ref{lem::3}}, $c \in G$, so $\mathcal{C}_{obst}^{min} \subset G$. Hence, $\mathcal{C}_{obst}^{min} = G$.
\end{proof}
% Intuitively, every $C_{obst}^{min}$ is a homeomorphism to $C_{obst}^{\overline{min}}$~\cite{lavalle2006planning}. 

In realistic scenarios, high configuration resolution ($c_c$, $c_m$, and $c_g$ are very close to each other) makes the area of $\mathcal{C}_{obst}^{min}$ very small. Real-world obstacle footprint (not arbitrarily small) are mostly larger than the area of $\mathcal{C}_{obst}^{min}$. Furthermore, when we instantiate $C_{obst}$ as discrete LiDAR beam ranges, the difference between different $C_{obst}^{min}$ is negligible. Therefore, we use one minimal unreachable set, $C_{obst}^{\overline{min}}$, which is all configurations along the straight line $c_m$ and $c_m'$ (the reflective symmetry point of $c_m$ with respect to $c_c-c_g$) to approximate all $C_{obst}^{min}$ ($C_{obst}^{\overline{min}}$ in Fig. \ref{fig::c_obst^min}). 

% Note that an accurate analytical representation of the $\mathcal{C}_{obst}^{min}$ boundary on the $c_m'$ side is actually a half ellipse whose focal points locate at $c_c$ and $c_g$, and whose semi-major axis is $(|c_c c_m'|+|c_m'c_g|)/2$, instead of a simplified half polygon (triangle). As shown in the right of the dashed line in Fig. \ref{fig::c_obst^min}, $c$ actually needs to be confined within the area defined by the half ellipse and the triangle, because any $c$ within the half ellipse will have a shorter $|c_cc|+|cc_g|$ than $|c_cc_m'|+|c_m'c_g|$. But with high configuration resolution, the area of the half ellipse and triangle becomes small, whose difference becomes negligible. This justifies the \textbf{symmetry assumption}.

\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{content/figures/c_obst^min5.png}
  \caption{
  $C_{obst}^{min_1},~C_{obst}^{min_2},~C_{obst}^{min_i},~...,~C_{obst}^{\overline{min}} \in \mathcal{C}_{obst}^{min}$. 
}
  \label{fig::c_obst^min}
\end{figure}

\subsection{Realistic Nonholonomic Robot}
\label{sec::realistic_robot}
Based on the principles discussed in Sec. \ref{sec::point_robot}, we present the hallucination technique for a realistic robot. In realistic scenarios, we approximate all $C_{obst}^{min}$ in $\mathcal{C}_{obst}^{min}$ with $C_{obst}^{\overline{min}}$. 

A realistic robot cannot be modeled as a simple point mass: (1) the size is not negligible and (2) it cannot change motion direction instantly. The former causes a difference in the robot workspace and C-space, while the latter introduces nonholonomic motion constraints. To address (1), we define one point to the left and another to the right of the centroid of the robot, offset by the robot width, as footprint points, shown in Fig. \ref{fig::real_robot}. The instant linear velocity along the line between these two footprint points is zero for nonholonomic vehicles. The polygon defined by a sequence of footprint points must belong to free space. The actual path executed by the optimal plan $p$ locates in the middle of this area. To address (2), we define $c_{\omega}$ as configurations between current and goal with a non-zero angular velocity ($\omega \neq0$). Given current, each $c_\omega$, and each $c_\omega$'s next configuration, their left or right footprint points are treated as $c_c$, $c_m$, and $c_g$ in the \emph{point robot} case: based on the sign of $\omega$, the robot turns left or right, and the left or right footprint points are chosen. 
For each triple of \emph{point robot} $c_c$, $c_m$, and $c_g$, we perform the same operations as in Fig. \ref{fig::c_obst^min}. 
% Since a real robot path is dense, the area defined by those points ($\mathcal{C}_{obst}^{min}$) is small, compared to the size of real-world obstacles. 
For simplicity and efficiency, we approximate all different $C_{obst}^{min}$ with $C_{obst}^{\overline{min}}$ for each triple. For a realistic optimal plan $p$ with \emph{actual} $c_c$ (current) and $c_g$ (goal) and multiple \emph{point robot} $c_c-c_m-c_g$ triples in between, we define the union of all $C_{obst}^{\overline{min}}$ as $\mathcal{C}_{obst}^{\overline{min}}$. 
In particular, we define an ``opposite'' function of $f(\cdot)$: 
$\mathcal{C}_{obst}^{\overline{min}} = o(p~|~c_c, c_g)$
as the \emph{minimal} hallucination function\footnote{Note the inverse function $f^{-1}(\cdot)$ does not exist. Technically, $c_g$ can be uniquely determined by $p$ and $c_c$, but we include it as an input to $o(\cdot)$ for notational symmetry with $f(\cdot)$.}. This function finds $\mathcal{C}_{obst}^{\overline{min}}$ based on the fact that  $p$ is an optimal plan. 

% In addition to the small area in the case of realistic robot model, because $C_{obst}^{min}$ is instantiated in terms of discrete LiDAR range readings, the difference between different $C_{obst}^{min}$ and $C_{obst}^{\overline{min}}$ further diminishes, as visualized in Fig. \ref{fig::real_robot}. 
As visualized in Fig. \ref{fig::real_robot}, $C_{obst}$ is instantiated in terms of discrete LiDAR range readings. 
For each LiDAR beam, we define a minimum and a maximum range, which limit the possible range readings of this particular beam based on the optimal plan $p$. The minimum range of all beams is determined by the left and right boundaries, as configurations within the boundary must be in $C_{free}$. We project all $C_{obst}^{\overline{min}}$ onto the corresponding LiDAR beams and for the beams directly intersect any $C_{obst}^{\overline{min}}$, the maximum range is set as the distance from the robot to the intersection point. For other beams, the maximum range is simply the LiDAR's physical limit, or manually pre-processed to a certain threshold. 
% A visualization of the LiDAR beams is shown in Fig. \ref{fig::real_robot}. 


\begin{figure}
  \centering
  \includegraphics[width=1\columnwidth]{content/figures/real_robot2.png}
  \caption{Applying the point robot example to realistic robot case: $C_{obst}^{min}$ is instantiated as LiDAR beams whose maximum is determined by ray casting.}
%   Due to high configuration resolution and discrete LiDAR beams, $C_{obst}^{\overline{min}}$ can efficiently approximate different $C_{obst}^{min}$.
  \label{fig::real_robot}
\end{figure}

\subsection{Sampling between Min and Max Range}
\label{sec::sampling}
Given a LiDAR scan with a minimum and maximum range for each beam, a sampling strategy is devised to create many obstacle sets, $C_{obst}$, in which $p$ is optimal. 
% The LiDAR beams with equal min and max values correspond to $C_{obst}^{\overline{min}}$, and are therefore fixed. Those are the reason why $p$ is optimal for shortest path. Other beams with different min and max values are called flexible beams, and their actual values are not crucial in determining if $p$ is optimal. 

Our sampling strategy aims at creating different range readings that (1) resemble real-world obstacles, and (2) respect uncertainty/safety. For (1), most real-world obstacles have a certain footprint, and their surface contribute to continuity among neighboring beams. Starting from the first beam, a random range is sampled between min and max with a uniform distribution. Moving on to the neighboring beam, with a probability $\alpha$, we increase, or decrease, the previous range by a small random amount, and assign the value to the current beam. This is to simulate the continuity in neighbouring beams. We make sure this value is within the min and max range of that beam. With probability $1-2\alpha$, we start from scratch and randomly sample between this beam's min and max values. This is to simulate the scenarios where the next beam misses the current obstacle, and reaches another one or does not reach any obstacle at all. For (2), we add an offset value as a function of the optimal plan $p$ to the ranges, for example, based on the speed of $p$. The rationale is that faster motion is correlated with more uncertainty or less safety, therefore only when the obstacles are far away from the robot, the optimal planner is confident to accelerate. 
% We also apply this offset to the fixed beams, because a good planner should not ``cut corners" aggressively. 

The entire HLSD pipeline is described in Alg. \ref{alg::sober}. The input to the algorithm is a random exploration policy $\pi_{rand}$ in open space, the minimal hallucination function $o(\cdot)$, a \emph{sampling count} of hallucinated $C_{obst}$ to be generated per raw data, the \emph{offset}$(\cdot)$ function, the probability $\alpha$, and a parameterized planner $f_{\theta}(\cdot)$. For every data in $\mathcal{D}_{raw}$ collected using $\pi_{rand}$ in open space (line 2), we hallucinate $\mathcal{C}_{obst}^{\overline{min}}$ (line 5) and generate the min and max values for every LiDAR beam (line 6). Lines 8--15 correspond to the sampling technique to generate random laser scans. We instantiate $C_{obst}$ as LiDAR readings $L$ and add it to $\mathcal{D}_{train}$ (line 16). This process is repeated \emph{sampling count} times for every data in $\mathcal{D}_{raw}$. Finally, we train $f_{\theta}(\cdot)$ with supervised learning (line 19). This hallucinated learning enables sober deployment with real perceived configuration $C_{obst}^{real}$ without runtime hallucination (Lines 21--22).

\begin{algorithm}[htbp]
 \caption{Hallucinated Learning and Sober Deployment}
 \begin{algorithmic}[1]
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 %\renewcommand{\algorithmicensure}{\textbf{Output:}}
 \REQUIRE $\pi_{rand}$, $o(\cdot)$, \emph{sampling count}, \emph{offset}($\cdot$), $\alpha$, $f_{\theta}(\cdot)$
\\\hrulefill
  \STATE // \textbf{Hallucinated Learning}
  \STATE collect motion plans $\{p, c_c, c_g\}$ from $\pi_{rand}$ in free space and form raw data $\mathcal{D}_{raw} = \{p, c_c, c_g\}$ 
  \STATE $\mathcal{D}_{train} \leftarrow \emptyset$
  \FOR {every $\{p, c_c, c_g\}$ in $\mathcal{D}_{raw}$}
  \STATE hallucinate $\mathcal{C}_{obst}^{\overline{min}} = o(p~|~c_c, c_g)$
  \STATE generate LiDAR range $L_{min}$ and $L_{max}$ with $\mathcal{C}_{obst}^{\overline{min}}$
    \FOR {iter = 1 : \emph{sampling count}}
    \STATE $L \leftarrow \emptyset$
    \STATE $l^1 \sim [l_{min}^1, l_{max}^1]$, $l^1 \leftarrow l^{1} + \text{\emph{offset}}(p)$
    % sample $l^1$ uniformly between $l_{min}^1$ and $l_{max}^1$
    \STATE add $l^1$ to $L$, $l^{last}\leftarrow l^1$
    \FOR{i = 2 : $|L|$}
        \STATE increase, decrease $l^{last}$ by a randomly selected small amount, or $l^i \sim [l_{min}^i, l_{max}^i]$, $l^i \leftarrow l^{i} + \text{\emph{offset}}(p)$, 
        % sample uniformly between $l_{min}^i$ and $l_{max}^i$, 
        with probability $\alpha$, $\alpha$, and $1-2\alpha$, respectively, and assign to $l^i$
        \STATE make sure $l^i \in [l_{min}^i, l_{max}^i]$
        \STATE add $l_i$ to $L$, $l^{last}\leftarrow l^i$
    \ENDFOR
    \STATE $C_{obst} \leftarrow L$, add $\{C_{obst}, p, c_c, c_g\}$ to $\mathcal{D}_{train}$
    \ENDFOR
  \ENDFOR
%   \STATE sample $\mathcal{D}_{raw}$ to generate a larger training set $\mathcal{D}_{train} = \{C_{obst}, p, c_c, c_g\}$, where $p=f(C_{obst}~|~c_c, c_g)$
  \STATE train $f_{\theta}(\cdot)$ with $\mathcal{D}_{train}$ by minimizing the error $\mathbb{E}_{(C_{obst}, p, c_c, c_g) \sim \mathcal{D}_{train}} \big[ \ell(p, f_\theta(C_{obst}~|~c_c, c_g))\big]$
\\\hrulefill
  \STATE // \textbf{Sober Deployment} (each time step)
  \STATE receive $C_{obst}^{real}, c_c, c_g$
  \STATE plan $p = \{u_i\}_{i=1}^{t} = f_{\theta}(C_{obst}^{real}~|~c_c, c_g)$
 \RETURN $p$
 \end{algorithmic}
 \label{alg::sober}
 \end{algorithm}



